Telling Left from Right: Learning Spatial Correspondence of Sight and Sound

Self-supervised audio-visual learning aims to capture useful representations of video by leveraging correspondences between visual and audio inputs. Existing approaches have focused primarily on matching semantic information between the sensory streams. We propose a novel self-supervised task to leverage an orthogonal principle: matching spatial information in the audio stream to the positions of sound sources in the visual stream. Our approach is simple yet effective. We train a model to determine whether the left and right audio channels have been flipped, forcing it to reason about spatial localization across the visual and audio streams. To train and evaluate our method, we introduce a large-scale video dataset, YouTube-ASMR-300K, with spatial audio comprising over 900 hours of footage. We demonstrate that understanding spatial correspondence enables models to perform better on three audio-visual tasks, achieving quantitative gains over supervised and self-supervised baselines that do not leverage spatial audio cues. We also show how to extend our self-supervised approach to 360 degree videos with ambisonic audio.

==> sections/ambisonic.tex <==
\section{Spatial Alignment in 360-Degree Video} \label{sec:ambisonics}

In the previous sections, we proposed a novel audio-visual correspondence task based on detecting spatial alignment between visual and audio streams, focusing on the more standard case of two-channel stereo audio with field-of-view vision. However, our method can also be applied to other types of videos, such as 360-degree video with full-sphere first-order ambisonics.  

\subsection{Problem Formulation}
First-order ambisonics (FOA) extends stereo audio to the 3D setting, with additional channels to capture sound depth and height: $a(t) = (a_w(t), a_y(t), a_z(t), a_x(t))$ where $a_w(t)$ represents the omnidirectional sound pressure, and $a_y(t), a_z(t), a_x(t))$ are the front-back, up-down, and left-right sound pressure gradients respectively. FOA is captured using a sound-field microphone and is often provided with 360-degree video to give viewers a full-sphere surround image and sound experience. Analogous to the case of stereo audio, we can train a model to detect whether the visual and audio streams are spatially aligned in 360-degree videos. To generate misaligned examples, we use the transformation, 
\begin{align}
\begin{split}
   \tilde{a}(t) = (&a_w(t), \\ 
   &a_x(t)\sin{\theta} +  a_y(t)\cos{\theta}, \\ 
   &a_z(t), \\ 
   &a_x(t)\cos{\theta} -  a_y(t)\sin{\theta}),
\end{split}
\end{align}
which rotates the spatial audio $a(t)$ about the z-axis by $\theta$, where $\theta \in [0.95*\pi, 1.05*\pi]$.

\subsection{Implementation Details}

We generally use the same model structure as the one we used for field-of-view video and stereo audio, as depicted in Figure \ref{fig:architectures}: the model consists of distinct visual and audio sub-networks that are fused prior to classification, and we reduce and flatten the visual features prior to fusion with the audio. The main difference is that the audio input is four channels instead of two. We train our model on the YouTube-360 dataset consisting of 360-degree videos with first-order ambisonics (FOA) audio \cite{Morgado18}. The dataset consists of over a thousand 360-degree videos with corresponding spatial audio, containing a variety of content including street views and musical performances. We use 3 second video clips sampled from full-length videos, introducing negative (rotated audio) examples with probability 0.5. We use 360-degree videos sampled at 5Hz with frames (as equirectangular projection) resized to 240 x 480. To augment the dataset, we randomly shift the color/contrast of the videos and apply random rotation about the z-axis of both video (via translation of the equirectangular projection) and spatial audio. For the W-channel, we use the short-time Fourier transform of audio sampled at 16kHz, and for the other channels, we take the inner product of the STFT with the W-channel STFT, which is an effective input for spatial audio localization tasks using neural networks \cite{Cao2019}.

\subsection{Results}

The results of the spatial alignment task trained on YouTube-360 dataset are shown in Table \ref{table:pretext-360}. As a baseline, we first initialized our visual sub-network using weights obtained from pretraining on ImageNet classification. We found that our model with visual sub-network trained from scratch performed comparably to this supervised baseline. Compared to earlier spatial alignment on the YouTube-ASMR and FAIR-Play datasets, these accuracy values appear low. We hypothesize that this is due to the more in-the-wild nature of the YouTube-360 dataset, resulting in sparser signals. On the other hand, we find that a model with only $60\%$ classification accuracy on 3-second clips does align 360-degree videos with high accuracy when evaluated over the entire video (approximately $~19$ degrees of rotational error for high confidence videos).

\begin{table}[h]
\begin{center}
\begin{tabular}{|l|c|}
\hline
Model & Test Accuracy \\
\hline
ResNet-18 (Supervised) & 0.57791 \\
\hline
No W-Channel & 0.61395 \\
No XYZ-Channels & 0.49535 \\
\hline
ResNet-18 & 0.58605 \\
\hline
\end{tabular}
\end{center}
\caption{Performance on pretext task: YouTube-360 dataset. The models perform comparably except the XYZ-channel ablation that eliminates spatial information.}
\label{table:pretext-360}
\end{table}

\iffalse
\subsubsection{Audio-Visual Spatial Alignment in 360 videos}
Manually aligning a spatial audio microphone with a 360-degree camera requires technical expertise, limiting the number of 360-degree videos produced with spatial audio. Our model for detecting audio-visual spatial misalignment is directly applicable to the task of correcting the spatial alignment of 360-degree videos. Specifically, for each video in the YouTube-360 test dataset, we compute the output of our model for uniform rotations of the spatial audio around the z-axis over multiple sub-sampled clips per video. We use consensus scoring to generate probabilities for different rotation angles and then compute the absolute value of the alignment error weighted by these probabilities. The results are shown in Table \ref{table:av-alignment}. 

\begin{table}[h]
\begin{center}
\begin{tabular}{c|c c c }
\hline
 & \multicolumn{3}{c}{Alignment Error (Degrees)} \\
Model & Low Conf & Med Conf & High Conf \\
\hline
Original & 65.34 & 50.51 & 19.06 \\
\hline
Shorter clips & 71.05 & 55.23 & 38.21 \\
Harder negatives & 74.69 & 66.65 & 47.00 \\
\hline
Direct prediction & ? & ? & ? \\
\hline
\end{tabular}
\end{center}
\caption{Comparison of different pretext models on AV alignment in 360-degree videos.}
\label{table:av-alignment}
\end{table}

Our model for detecting audio-visual spatial misalignment performs well on this task, with high confidence predictions achieving a weighted error of $19$ degrees. \textcolor{red}{Comment on directly predicting the angle of misalignment.} Interestingly, making the pretext detection task more challenging (i.e. decreasing the clip length or increasing the difficulty of the negative examples) did not improve downstream performance on this task. \textcolor{red}{Brief discussion.}
\fi


\section{Analysis and Evaluation of Features}
\subsection{Sound Localization}
%Analogous to our earlier results using videos with stereo audio, we find that the audio sub-network trained on this generalized form of the spatial alignment task learns meaningful spatial audio cues. Specifically, the first two principal components of the audio embeddings extracted from held-out data successfully localize sound sources to the X-Y plane, and we can visualize the location of sound sources in the 360-degree video based on the audio alone (Figure \ref{fig:360-spatial-pca}).
%While we could focus on 
Sound localization based on microphone array data and/or first-order ambisonics is a particular interesting problem in itself. Traditionally, the direction-of-arrival (DOA) of sound signals is computed using beamforming algorithms by sampling many points along the sphere, computing the energy that arrives from each direction, and choosing the direction with maximal energy. However, these methods generally only handle individual sound signals and do not take timbre information into account. In recent years, deep learning models have emerged for simultaneously classifying sound events and determining their direction-of-arrival. To our knowledge, these methods have so far only relied on strong supervision for training. While there is relatively more labeled data available for sound event classification, there is a scarcity of in-the-wild sound events labeled with their direction-of-arrival. This latter type of data is challenging to collect and is therefore almost always synthetically generated by panning sound events in a fixed number of directions.

As shown in Figure \ref{fig:360-spatial-pca}, our audio sub-network convincingly extracts spatial cues from in-the-wild spatial audio in a self-supervised manner, which can be visualized over the video similar to Section \ref{sec:sound-source-loc}. To determine whether this pretrained network provides a quantitative boost on spatial audio localization tasks, we evaluated the learned audio representation on the Tau Spatial Sound dataset \cite{adavanne2019multi}. This dataset consists of 400 minute-long recordings of multiple sound events synthetically up-mixed to 36 different directions along the X-Y plane (every 10 degrees). In the 2019 DCASE Sound Event Localization and Detection challenge, participants were asked to output the class and direction of the arrival of these sound events. All of the models were trained from scratch in a strongly-supervised manner.

To evaluate the quality of our pretrained audio features, we conducted two experiments on this dataset. First, we compared an audio classification network trained from scratch with one that was initialized using the weights from our pretrained audio sub-network. We found that our pretrained weights provided a considerable boost over the baseline in the prediction of direction of arrival (Table \ref{table:dcase-doa}). Second, we extracted the embeddings of the Tau Spatial Sound audio clips using our pretrained audio sub-network and performed classification using a linear SVM, providing only one example of an event from each direction of arrival (one-shot learning). Even in this case, we were able to predict the direction of arrival with a mean error of only ~30 degrees. These results suggest that the spatial information extracted using our self-supervised task are strongly useful for acoustic localization.

\begin{table}[h]
\begin{center}
\begin{tabular}{|c|c|}
\hline
Method & Mean Error \\
\hline
Trained from scratch & 20.5 $\pm$ 1.17 \\
Pretrained weights & 17.5 $\pm$ 0.62 \\
\hline
One-shot SVM on random embeddings & 78.6 \\
One-shot SVM on our embeddings & 29.5 \\
\hline
\end{tabular}
\end{center}
\caption{Performance on DCASE 2019 DOA estimation (azimuth angle). Error shown is mean prediction error in degrees (lower is better, maximum is 180, random is 90). Standard deviation shown is based on 4-fold cross validation sets. }
\label{table:dcase-doa}
\end{table}

\begin{figure*}[t]
\begin{center}
   \includegraphics[width=0.65\linewidth]{figures/yt360-pca.png}
   \includegraphics[width=0.25\linewidth]{figures/tau-pca.png}\\
   \vspace{0.5cm}
   \includegraphics[width=0.8\linewidth]{figures/yt-acoustic-loc-demo.png}
\end{center}
   \caption{(a) PCA plots of YouTube-360 audio embeddings. (b) PCA plot of Tau Spatial Sound dataset. (c) Visualization of predicted sound locations based on audio only overlaid on Youtube-360 videos}
\label{fig:360-spatial-pca}
\end{figure*}

